Self-Improving LLM Agents at Test-Time

One paradigm of language model (LM) fine-tuning relies on creating large training datasets, under the assumption that high quantity and diversity will enable models to generalize to novel tasks after post-training. In practice, gathering large sets of data is inefficient, and training on them is prohibitively expensive; worse, there is no guarantee that the resulting model will handle complex scenarios or generalize better. Moreover, existing techniques rarely assess whether a training sample provides novel information or is redundant with the knowledge already acquired by the model, resulting in unnecessary costs. In this work, we explore a new test-time self-improvement method to create more effective and generalizable agentic LMs on-the-fly. The proposed algorithm can be summarized in three steps: (i) first it identifies the samples that model struggles with (self-awareness), (ii) then generates similar examples from detected uncertain samples (self-data augmentation), and (iii) uses these newly generated samples at test-time fine-tuning (self-improvement). We study two variants of this approach: Test-Time Self-Improvement (TT-SI), where the same model generates additional training examples from its own uncertain cases and then learns from them, and contrast this approach with Test-Time Distillation (TT-D), where a stronger model generates similar examples for uncertain cases, enabling student to adapt using distilled supervision. Empirical evaluations across different agent benchmarks demonstrate that TT-SI improves the performance with +5.48% absolute accuracy gain on average across all benchmarks and surpasses other standard learning methods, yet using 68x less training samples. Our findings highlight the promise of TT-SI, demonstrating the potential of self-improvement algorithms at test-time as a new paradigm for building more capable agents toward self-evolution.

==> sections/6-ethics_statement.tex <==
\section*{Ethics Statement}
This research investigates test-time self-improvement (TT-SI) for language-based agents using publicly available benchmarks.
No personally identifiable information or sensitive human data was collected or used. All experiments rely on synthetic datasets, open-source corpora, or established evaluation benchmarks. 
We recognize potential risks, such as biases from LLM-based data generation and training, which are mitigated by the nature of test-time training (TTT), as we do not store any model weights.
We further mitigate these by (i) reporting transparent experimental details, (ii) restricting scope to controlled research settings, and (iii) emphasizing reproducibility and responsible use. Our research adheres to the ICLR Code of Ethics by prioritizing fairness, privacy, and scientific integrity.


==> sections/8-llm_statement.tex <==

\section*{Use of LLMs}
LLMs were used in this work for three purposes: (i) as base models under study for test-time training, (ii) as baselines for empirical comparison, and (iii) for minor assistance in refining the readability of this manuscript. Both open-source (e.g., Qwen~\citep{yang2025qwen3}) and closed-source models (e.g., GPT-5-mini\footnote{\url{https://platform.openai.com/docs/models/gpt-5-mini}}) were employed for training and data-generation. 
The prompt used for improving writing quality was similar to \textit{"Please make more clear sentence, making sure to remove any grammatical mistakes."}
Importantly, all scientific ideas, methods, experiments, and conclusions originate from the authors. When LLMs were used for language refinement, outputs were carefully reviewed to prevent the introduction of hallucinated or incorrect content, ensuring that all arguments, findings, and perspectives are solely those of the authors.

